Radiative $b\to d$ Penguins

This article gives an overview of the recent searches and measurements of $b\to d$ penguin transitions with the BaBar experiment. The branching fraction of these decays in the Standard Model (SM) is expected to be a factor of 10 or more lower than the corresponding $b\to s$ penguin transitions, but a deviation from the SM prediction would be an equally striking sign of new physics. The exclusive decay $B\to\pi\ell\ell$ is searched by BaBar with no excess over the background found. The BaBar measurement of $B\to(\rho,\omega)\gamma$ provides the first evidence of $B^+\to\rho^+\gamma$, is in good agreement with the previous Belle results and provides a measurement of $|V_{td}/V_{ts}|$ independent of the one from $B_s$ mixing. No deviation from the SM is found.

==> makefile <==
LATEX = latex
DVIPS = dvips
MF = mf
#-----------------------------------------

TEX_MAIN=PBe_MoriondEW07
TEX_FILES=$(TEX_MAIN).tex
PICTURES=figures/*.eps
MF_ARGS='\mode:=localfont; input fmftempl'
date=`date +%Y%m%d`

#-----------------------------------------
TARGET=all

all: $(TEX_MAIN).ps

.PHONY=tar

#-----------------------------------------
$(TEX_MAIN).dvi: $(TEX_FILES) $(PICTURES)
	-rm *.mf *.t1 *.tfm *.*pk *.*gf
	-$(LATEX) $(TEX_MAIN)
	$(MF) $(MF_ARGS)
	-$(LATEX) $(TEX_MAIN)
	-$(LATEX) $(TEX_MAIN)

$(TEX_MAIN).ps: $(TEX_MAIN).dvi
	$(DVIPS) $(TEX_MAIN)

$(TEX_MAIN).pdf: $(TEX_MAIN).ps
	ps2pdf -sPAPERSIZE=a4 $(TEX_MAIN).ps

tar: $(TEX_MAIN).pdf
	tar cvfz $(TEX_MAIN)_$(date).tgz *.tex *.ps *.pdf makefile figures/*.eps figures/*.epsi figures/*.fig *.cls *.sty figures/*.ps

clean: 
	rm *.log *.dvi *.aux *.mf *.t1 *.tfm *.*pk *.*gf *.pdf

